TSoR: TCP Socket over RDMA Container Network for Cloud Native Computing

Cloud-native containerized applications constantly seek high-performance and easy-to-operate container network solutions. RDMA network is a potential enabler with higher throughput and lower latency than the standard TCP/IP network stack. However, several challenges remain in equipping containerized applications with RDMA network: 1) How to deliver transparent improvements without modifying application code; 2) How to integrate RDMA-based network solutions with container orchestration systems; 3) How to efficiently utilize RDMA for container networks. In this paper, we present an RDMA-based container network solution, TCP Socket over RDMA (TSoR), which addresses all the above challenges. To transparently accelerate applications using POSIX socket interfaces without modifications, we integrate TSoR with a container runtime that can intercept system calls for socket interfaces. To be compatible with orchestration systems like Kubernetes, TSoR implements a container network following the Kubernetes network model and satisfies all requirements of the model. To leverage RDMA benefits, TSoR designs a high-performance network stack that efficiently transfers TCP traffic using RDMA network. Thus, TSoR provides a turn-key solution for existing Kubernetes clusters to adopt the high-performance RDMA network with minimal effort. Our evaluation results show that TSoR provides up to 2.3x higher throughput and 64\% lower latency for existing containerized applications, such as Redis key-value store and Node.js web server, with no code changes. TSoR code will be open-sourced.

==> abstract.tex <==
% Serverless container computing is a popular cloud computing paradigm which enables cloud users to run containers while abstracts away the management of actual servers or computing infrastructure where containers are running on. Serverless container computing needs a container network which is not only highly performant but also needs support multi-tenant network traffic isolation, higher scalability and fast container startup and tear down. We have designed and implemented a new serverless container network,TCP Socket over RDMA (TSoR), which is a RDMA based multi-tenant container network based on secure container runtime Quark. TSoR uses RDMA as underlying data plane to transmit application TCP/IP traffic, supports multi-tenant isolation and provides Kubernetes network model compatible support such as container virtual IP, DNS based service discovery. We illustrate its power by showing by showing improvements (of 2-5× in latency and 9× in throughput, this should have some latest data) for existing containerized TCP/IP application without modification. 
Container network performance is crucial for cloud-native containerized applications. Meanwhile, RDMA offers higher throughput and lower latency networks.
Unfortunately, it has several challenges while empowering container networks with RDMA: 
1) Transparent improvements without modifications of applications
2) Integration with container orchestration systems

In this paper, we present TCP Socket over RDMA (TSoR), a RDMA based TCP/IP container network service for cloud native computing. 
TSoR achieves high performance as its data plane is based on the RDMA network;
TSoR provides POSIX socket interface for applications and transparently transfers TCP traffic over RDMA connection
so that existing containerized applications can use TSoR without modification; 
TSoR provides Kubernetes-compatible container network support and it is a turn key solution for existing Kubernetes cluster to adopt TSoR with minimal effort. 
We implement TSoR in open source secure container runtime Quark and evaluation results show that TSoR reduces up to 66\% latency with NPtcp benchmark and 2 times of throughput with Redis benchmark in comparison with host network.




==> architecture.tex <==
\section{Architecture}
TSoR has the following design goals:
\begin{itemize}
\item {\bf Performance improvement for TCP traffic}: TSoR is designed to leverage RDMA NIC to transmit TCP traffic. It should have increased throughput and decreased latency.
\item {\bf Transparency to the application programmer}: TSoR is designed to significantly improve performance without requiring modifications to applications or containerized image.
\item {\bf Multi-tenant isolation support}: TSoR is designed to support isolating network traffic between different tenants.
\item {\bf Fast container start up and tear down}: TSoR is designed to support serverless container computing which means container will be started and stopped frequently, fast container start up and tear down is a must.
\item {\bf Kubernetes network model compatibility}: TSoR is designed to be fully compatible with Kubernetes network model. There should be minimal effort to set up TSoR for existing Kubernetes cluster so that it can be used in existing Kubernetes ecosystem.
\end{itemize}
In this section, we show how we achieve these goals in TSoR. We describe the infrastructure requirement for this architecture, and we detail interface and design of the control plane and data plane of TSoR. Finally, we describe our implementation of TSoR based on secure container runtime Quark.

\subsection{Architecture Overview}

TSoR targets cluster which has RDMA network support. Figure 2 shows the overall architecture. TSoR control plane assign container IP, get nodes and containers information from Kubernetes API Server. TSoR data plane use information from control plane to set up RDMA connections between cluster nodes, established TCP connections and transfer TCP traffic using RDMA IB verbs. Traffic inside cluster using TSoR will leverage RDMA, TSoR gateways are introduced to transform traffic between TCP and RDMA when communicating with outside cluster entities.
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TSoRArchPlanes.png}
 \caption{TSoR Architecture}
%  \label{fig::arch}
 \end{figure}
\subsection{TSoR Interface}
There're 2 categories of interface when using TSoR:

{\bf 1. Application Programming Interface}

Applications still use normal POSIX socket API[] for TCP related operations. As socket API calls interception happens in Quark's system call virtualization layer, that means it doesn't need any code modification or rebuilding of application, even existing container image can use TSoR directly which provides transparency to application programmers. We believe POSIX socket API will be still be mainstream API as it's more friendly compared to IB verb programming.

{\bf 2. Kubernetes related interface}

TSoR supports Kubernetes networking model including container IP address assignment, service, DNS based service discovery and intra-cluster load balance so that TSoR can be applied to existing Kubernetes cluster with minimal effort.

\subsection{TSoR Control Plane}
TSoR control plane is responsible for container IP assignment, supporting Kubernets network model and talking to Kubernets API server to watch node and container information.

\subsection{TSoR Data Plane}
The main goal of TSoR is to provide a faster container network by transferring TCP traffic over the RDMA network. TSoR will intercept TCP socket system calls, create RDMA connection between TCP client and TCP server and transfer TCP data through the RDMA connection. Figure 3 shows an example data transfer process using TSoR. In this example, there are 2 Quark containers, i.e. Client application and Server application, are running on 2 bare-metal machines, i.e. Node1, Node2. There are RDMA networks available between them.  In the example scenario, the client application will use a TCP connection to send data to the server application. The underlying data sending process is as below.

\textbf{1. Sys\_send system call}: Client Application call system call sys\_send to ask OS kernel to send data in a user space buffer to Server Application;

\textbf{2. Memory copy from user space to OS kernel}: The Quark OS kernel takes over control through the sys\_send system call and copy the data from user space to the Quark kernel socket send buffer;

\textbf{3. RDMA data transfer}: As there is an RDMA network between the 2 nodes, the client Quark OS kernel will use RDMA IB verbs to write the data to the Server application’s Quark kernel socket recv buffer;

\textbf{4. Memory copy from OS kernel to user space}: After the data is written to the Server application Quark Kernel recv buffer, the server Quark kernel will copy it to the server application’s application recv buffer.

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/data_path.png}
 \caption{TSoR Data Plane}
%  \label{fig::arch}
 \end{figure}
 
As Figure3 shows, the interception of TCP socket releated calls happens at Quark System Call Virtualization layer so it's totally transparent to application.

\subsection{TSoR Gateway}
TSoR gateway will be used to bridge communication between inside and outside of clusters. In addition to standard Kubernetes gateway functionalities, TSoR gateway has its own special chanllenges which will be presented in section 4 design challenges.

==> backup/background_old.tex <==
\section{Background}

\subsection{Container Runtime}

\subsection{Container Network Interface (CNI)}
k8s model compatiable

\subsection{RDMA for Container, High Performance Network}
high-perf. network, transparent 



This section provides a brief background on serverless container computing, serverless container network, RDMA network, the Quark container runtime and the existing zero memory copy socket solutions. 

\subsection{Serverless container computing}
There are 2 kinds of serverless container service: Serverless Kubernetes service, e.g. GKE autopilot and serverless non-Kubernetes container service, e.g. Google Cloud Run. Based on serverless Kubernetes service, customers could get a virtual Kubernates cluster to run their pods without provision of a Virtual Machine cluster. Based on the serverless non-Kubernetes container service, customers could submit their container image and run them with on-demand invocation.

Both of the 2 serverless container services will run multi-tenant containerized workloads in a shared multi-tenant environment without pre-provision Virtual Machines.  As they don’t rely on Virtual Machine to do the computation isolation, they need to sandbox the container workload in a secure container runtime. There are 2 types of open source secure container runtime: Linux Kernel based container runtime such as Kata[], non-Linux Kernel secure container runtime, e.g. gVisor[] and Quark[]. Linux Kernel 
based container runtime sandbox container workload in a optimized Linux Kernel with Container Runtime Interface extension. The non-Linux Kernel secure container runtime implements a Linux compatible OS Kernel and a dedicated Virtual Machine Monitor (VMM). As it doesn’t depend on Linux Kernel, it is possible to extend functions which doesn’t supported by Linux Kernel on the non-Linux Kernel secure container. TSoR is an extension of the Quark container runtime.

Both of the 2 serverless container services need a serverless container network to isolate multi-tenant network traffic. The serverless Kubernetes service has more complex container network requirements than the non-Kubernetes container service and could be considered as a superset of that. So late we will only discuss the serverless container network for the serverless Kubernetes service. The TSoR is designed to support both of them.

\subsection{Serverless Container Network}
Serverless container network could be considered as a normal single tenant container network with multi-tenant support. In Kubernetes, the Kubernetes network model[] is defined for a container network. The network model defines the container communication for intra-pod, inter-pod and with outside of the cluster. Different container runtimes could implement the Kubernetes network model by providing a Container Network Interface (CNI) plugin. There are multiple container network CNI providers such as Flannel[], Calico[], Cilium[]. Serverless container networks need to support both the Kubernetes network model and the multi-tenant network isolation.

\subsection{RDMA}
The Remote Direct memory Access (RDMA) allows one application to access another application memory running in another machine directly and bypass the OS Kernel. It could achieve lower latency and high throughput with less CPU consumption []. The RDMA network has been enabled in cluster infrastructure and supports data intensive applications such as machine learning and HPC.

There are multiple ways to expose the RDMA interface to the container. SR-IOV[] is a hardware based solution and Freeflow[] is a software based solution.

There are also some solutions to transfer the TCP traffic through RDMA. The common idea of them is to intercept TCP socket system calls, set up a RDMA connection based on the sys\_connect target ip address and then transfer the data through the RDMA connection. SMC[] intercept the TCP socket system call by changing Linux Kernel and DirectSocket[] intercept system call with LD\_PRELOAD. The TSoR intercepts the TCP socket in Quark runtime.

% \subsection{Quark container runtime architecture }
% Quark[] is a secure container runtime. It could be considered as a virtual OS kernel designed to run on Linux host space. The Quark architecture is as below. Unlike the common Linux Virtual Machine design, VMM, e.g. qemu, will virtualize the computer device and support different virtual machine OSes like Linux and Windows, Quark’s VMM QVisor only supports its virtual OS Kernel QKernel. The QKernel simulates the system calls with Linux kernel semantics on the underlying Linux host kernel. By default Quark intercept TCP socket system calls and  transfers the TCP traffic through the underlying container network over the host TCP/IP protocol stack. Instead, TSoR added another RDMA based  protocol stack which transfers the TCP data over RDMA connections.
% \begin{figure}[tbp]
%      \centering
%  \includegraphics[width=\linewidth]{graphs/charts/QuarkArch.png}
%  \caption{Quark Architecture}
% %  \label{fig::arch}
%  \end{figure}

% \subsection{Zero Memory Copy Socket
% }
% Memory copy between user space and OS Kernel is a well known performance overhead for BSD Socket. There are some solutions [][] addressing this issue. But the solutions are not suitable for RDMA based TCP data transfer. For example, MSG\_ZEROCOPY will lock the user space buffer when doing sys\_sendmsg. But RDMA requires pre-register data buffer and registering a new buffer for each sys\_sendmsg will increase latency. Zero-copy TCP receive[] will map the socket’s kernel receive buffer to user space. It has limitations that Mapping of memory into a process's address space is done on a per-page granularity. And it needs to do sys\_mmap for each sys\_recvmsg whose performance overhead is high as it might lead to TLB shootdown.





==> backup/introduction_old.tex <==
\section{Introduction}
Serverless container computing is becoming a more and more popular cloud computing paradigm. Based on that, users can run microservices in their containers in a serverless environment. It has been supported by major cloud providers such as AWS Fargate/EKS on Fargate \cite{fargate}, Google Cloud run\cite{googlerun}/GKE autopilot\cite{gkeautopilot}, Azure Container Instance\cite{azurecontainer}/AKS virtual Node\cite{AKSvirtualNod}.

Serverless container computing will run multi-tenant containerized service in a shared environment to handle on-demand user requests. To isolate computation between tenants,  it requires a secure container runtime with Virtual Machine level computation isolation. To handle on-demand user requests, it requires high density deployment and high frequency container startup and tear down to support user application latency request response. As multiple tenants' workloads are running in one environment, it has more scalable requirements than single tenant contain computing.

Serverless container computing also needs a severless container work to provide a multi-tenant network. In addition to single tenant Container Network’s the existing high throughput and low latency demonding, the serverless container network has more requirement:

\textbf{Multinenant isolation}: Serverless container network needs to isolate network traffic between different tenants. Each tenant should have its dedicated network namespace like a virtual machine VPC network.

\textbf{High scalability}: In serverless container environments, multiple tenant containers are running in one shared environment. Furthermore, a serverless container might have smaller resource requirements than a common microservice container so that it has high deployment density. So it needs to support more containers than a single tenant container network.

\textbf{High throughput \& low latency container IP address assign/reclaim}: Serverless container computing needs to support on-demand requirement invocation, so the containers will frequently startup and tear down. To support that, the serverless container network needs to frequently assign/reclaim ip addresses for containers and propagate the ip addresses route information across the cluster.

Network performance is always the requirement for container networks. Most of the state-of-the-art container networks such as Flannel\cite{Flannel},... are based on TCP/IP protocol stack with overlay or underlay solution. They are using different technology to improve the performance such as eBPF, xDP, DPDK, NIC passthrough. As they provide another layer of virtualization over the TCP/IP protocol stack, most of their performance’s up-limite is host TCP/IP  network.

RDMA networking offers significantly lower latency, higher throughput with lower CPU consumption than TCP/IP based protocol stack. RDMA has been widely deployed in cloud environments to support data-intensive applications such as machine learning, High Performance Computing (HPC). Besides Infiniband, RDMA can also run over or ethernet (RoCE) which is widely available in common cloud clusters. It is a charming idea to build a container network over RDMA to support microservice communication and achieve  higher performance.

There are 3 challenges to transfer cloud native microservice network traffic over RDMA in a serverless environment:

\textbf{TCP socket compatibility}:  The existing cloud natice microservers are using TCP/IP based RPC such as http/gRPC which accesses the network infrastructure through BSD socket system calls. The RDMA’s programing interface, i.e. the IB verb, is totally different from socket. The cost is high to migrate existing microservice to RDMA.

\textbf{Virtual container network compatibility}: The cloud services depend on the container network’s virtualization functions to work, such as virtual container IP address, DNS based service discovery and intra-cluster load balance. RDMA has no such native virtualization support.

\textbf{Multi-tenant network isolation}: Serverless container networks are required to isolate network traffic of different tenants. The native RDMA data plane bypasses the OS Kernel and has limited network namespace level isolation. and it is hard to isolate multi-tenant networks.

There are some solutions to transparently transfer TCP traffic over the RDMA network such as SMC\cite{SMCR}, SocketDirect\cite{li2019socksdirect}. SMC is changing the Linux OS Kernel to intercept TCP traffic. SocketDirect is using LD-Preload intercept TCP traffic. They partially solve the TCP based application’s RDMA compatibility issue. But they don’t address the second and third challenges.

There are also some solutions to expose the RDMA interface to containers such as Freeflow\cite{kim2019freeflow}. Freeflow is a virtual RDMA networking framework to transparently expose native RDMA IB verbs into containers with resource sharing and isolation. It addresses the third challenge but doesn’t handle the first and second challenges.

In this paper, we present TCP Socket over RDMA (TSoR), a RDMA based serverless container network. It is implemented in the secure container runtime Quark\cite{Quark} and designed as a Kubernetes cloud network plugin provider with multi-tenant support. It has following characters:

\textbf{TCP socket compatible RDMA based TCP traffic transfer}: It provides a BSD socket compatible system call interface to intercept cloud native microservice TCP traffic and transfer the TCP data through the underneath RDMA connection. So existing containerized microservice can run over that without modification. And also can take advantage of RDMA network’s low latency, high throughput with less CPU consumption.

\textbf{Kubernetes container network compatibility}: It is designed as a Kubernetes container network plugin provider. It meets Kubernetes container network requirements which provides container virtual IP address assignment, DNS based service discovery and intra-cluster load balance etc.

The TSoR’s data plan is based on RDMA. It has better performance than the TCP/IP protocol stack, but it can’t reach native RDMA application’s performance. One of the major performance overheads is the well known BSD socket memory copy between user space and OS Kernel. TSoR also provides an attempted solution to address this issue.

\textbf{Zero memory copy TCP socket extension}: TSoR extends system call sys\_mmap to expose Quark kernel TCP ring buffers to user space and add 2 more system calls to enable user application to effectively get/set the ring buffers’ head/tail pointers. User applications can use this extension to achieve near native RDMA performance in the TSoR serverless container network. The feature is an extension to TCP socket and all the existing TCP socket features can still work. 

We evaluate the performance of TSoR with standard benchmark tools and real-world application benchmarks and compare the result with existing Container network Flannel in Kubernetes and different container runtimes including Runc, Quark and Kata. We also compare the result with runC on the host network. TSoR’s performance is better than Flannel in the majority scenario. And TSoR has much less latency than the host network. For the TSoR zero memory copy socket extension, as it has no standard benchmark or application support, we built a simple PingPong benchmark tool to compare the performance with native RDMA application and runC on the host network. The test result shows that it achieves near native RDMA results and much better than the host network.





==> design.tex <==
\section{Overview}
\subsection{Design Goal}
TSoR has the following design goals:
% \textbf{Design Goals / Motivation}:eo
\begin{itemize}
\item {\bf High performance container networking for micro-service}: TSoR is designed to transmit TCP traffic through RDMA connection which bypass TCP/IP protocol stack and host Linux kernel. So it achieves high throughput,  low latency with lower CPU consumption.

\item {\bf Transparency to the application programmer}: TSoR are based on POSIX socket interface. It is designed to significantly improve performance without requiring modifications to applications or containerized application image.

\item {\bf Self-contained container network plugin of Kubernetes environment}:  TSoR is designed to be fully compatible with Kubernetes network model. There should be minimal effort to set up TSoR for existing Kubernetes cluster so that it can be used in existing Kubernetes ecosystem. At the same time, TSoR supports multi-tenant network traffic isolation and provides an efficient network traffic routing solution to address frequent container start up and tear down in serverless computing.
\end{itemize}

\subsection{Requirement}

\zhao{new subsection title}

\zhao{formal explanation for network model }

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/requirement.png}
 \caption{TSoR Requirement}
%  \label{fig::arch}
 \end{figure}
TSoR is designed as a container network solution. It needs to provide follow connection as Figure\#\#: \circled{1} Intra-node Pod to Pod , \circled{2} Inter-node Pod to Pod , \circled{3} External to Pod (i.e. ingress), \circled{4} Pod to External.

The connection \circled{1} \circled{2}  are Kubernetes cluster internal connection, TSoR will provides a RDMA based TCP connection. The connection \circled{3} \circled{4} are external facing connection, TSoR needs to provide TSoR gateway to handle data transfer. 

\subsection{Design Challenge}

\zhao{new subsection title}

TSoR's goal is to use RDMA as data plan for container network internal TCP socket traffic. The semantic of TCP socket is to transmit data from a local buffer to its peer's remote buffer. RDMA NIC supports to copy data from an application local buffer to remote machine's application buffer with a reliable connection just like TCP connection. The major idea of TSoR data plane is the hardware offloading of the TCP traffic to RDMA NIC instead of through TCP/IP protocol stack.  

\zhao{major idea}

RDMA supports both unreliable and reliable connection. TSoR choose the RDMA Reliable Connection (RC) for TCP data transmission so that TCP/IP protocol stack work such as congestion control, re-transmission of lost packets is offloaded to RDMA NIC hardware. 

SMC[] and DirectSocket[] has done similar work. In their design, one TCP connection has one underlying RDMA Connection, i.e. Reliable Connection (RC) Queue Pair (QP). From TSoR initial Prove of Concept evaluation work, we found the performance issue for such one TCP connection to one RDMA Connection as below. 

\zhao{paraphrase}

\begin{itemize}
\item \textbf{RDMA Reliable Connection scalability}: In a typical cluster environment, the micro-services running on single bar-metal machine might need 1 million TCP connections. Per [], RDMA NIC \textbf{performance will decrease when its Reliable Connection count reach a few hundred}?. 

\zhao{unclear}

\item \textbf{RDMA connection setup latency}: The RDMA Connection establishment needs another communication channel, e.g. TCP, to help exchange QP metadata. We measured the latency of creating such RDMA Connection based on TCP and found the latency is about 5000 microsecond while a common TCP connection only take about 500 microseconds?. 
\end{itemize}

So it is not practicable for to map one TCP connection to one RDMA Reliable Connection.


\section{Architecture}

\zhao{New Section Title}

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TSoRArchv3.png}
 \caption{TSoR Architecture}
%  \label{fig::arch}
 \end{figure}
 
Figure 3 shows a TSoR cluster. It includes multiple Cluster Nodes and a Cluster Orchestration System, e.g. Kubernetes. The Cluster Nodes will connect with each other with RDMA Connection, i.e. RDMA Reliable Queue Pair. There are TCP ingress and egress traffic in TSoR cluster to communicated with external. 

Each Cluster Nodes will composes one RDMA Service, multiple Quark enabled Pods, and one TSoR Gateway.
\begin{itemize}
\item \textbf{RDMA Service}: RDMA Service is the TSoR's central component. It connects to Quark Pods, TSoR Gateway and the orchestration environment control plane, e.g. Kubernetes API Server. It is the only component access RDMA NIC in whole system;
\item \textbf{Quark Pod}: Quark Pod is a Kubernetes Pod running with Quark runtime integrated with TSoR. TSoR integrate with Quark Pod with TSoR Client. TSoR Client takes over the pod user application's TCP traffic intercepted by Quark runtime system virtualization layer and transmit it with RDMA Connection through RDMA Service. \zhao{Name for Quark Pod}
\item \textbf{TSoR Gateway}: TSoR cluster internal traffic is carried by RDMA network. But external traffic is using TCP/IP protocol. To bridge the TSoR internal pods with external, TSoR gateway is needed to do protocol transformation between TCP and RDMA for external facing traffic. TSoR Gateway will proxy the external TCP traffic to (ingress) or from (egress) Quark Pod through the RDMA Service. TSoR Gateway also used the TSoR Client to connect with the RDMA Service.
\end{itemize}
We will give detail introduction of RDMA Service, TSoR Client in the Quark Pod and TSoR Gateway.
\subsection{RDMA Service}
 
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/RDMASrv.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 
 

RDMA service is the TSoR's core component. Figure 4 shows its design. It has following sub components:

\begin{enumerate}
\item \textbf{RDMA Client Manager}: RDMA Client Manager maintains the client connections from Quark Pods and TSoR Gateway to RDMA service. The TCP traffic intercepted by Quark runtime and TSoR Gateway will be forwarded by the TSoR Client to RDMA Service through the Client Manager. The Client Manager use a Shared Memory Region (SHM Region) to share data with TSoR Client. The Shared Memory Region includes 2 components: a message queue pair and a Shared Buffers. 
\begin{enumerate}
\item \textbf{Message queue pair}: The message queue pair includes 2 shared memory queues: Submission Queue (sq) and a message Complete Queue (cq). The queues are lockless shared memory queue. TSoR Client will send request message to Client Manager through sq and recieve the response message from Client Manager through cq.
\item \textbf{Shared Buffers}: Share Buffers is a shared memory area. It has TSoR read/write data buffers to store TCP data. The TSoR read/write data buffer is a fixed size ring buffer. And TCP traffic data is stored in the ring buffer and shared between Quark Pod and RDMA Service. The TSoR data buffer is also the Memory Region (MR) which is pined (i.e. no Swapping) in host Linux Kernel. So that RDMA NIC can could read data from local Quark Pod TSoR write buffer and write it to remote peer Quark Pod's TSoR read buffer without memory copy.
\end{enumerate}
\item \textbf{RDMA Connection Manager}: The RDMA Connection Manager manages all the RDMA Connection (i.e. Reliable Connection Queue Pair) 's setup, tire down and data transmission. RDMA Service will setup a RDMA Connection to connect each other Cluster Node when it is startup. This is our solution to mitigate the issues described in section 3.2 as below:  
\begin{enumerate}
\item \textbf{RDMA Connection scalability}: All the TCP connection between the two Nodes will share the RDMA Connection. So the RDMA Connection count of single Node is about the Node Count of the cluster which is about hundreds or thousands. This count is much less than the TCP connection count which might reach one million. This mitigation enables TSoR to support a cluster with hundreds Nodes. We are working on the solution based on this to scale the cluster size to tens thousand Nodes. 
\item \textbf{RDMA connection setup latency}: As the RDMA Connections are setup when the RDMA Service startup, when there is TCP connection request coming, the RDMA Connection Manger could use the RDMA Connection to setup virtual TCP connection by exchanging virtual TCP connection metadata. As the RDMA latency is much less than TCP/IP protocol stack, TSoR can achieve low TCP connection setup latency. 
\end{enumerate}
\item \textbf{RDMA Control Plane Agent}: RDMA Service need get cluster level connection related metadata from TSoR cluster control plane, e.g. Kubernetes API Server in Kubernetes cluster. The connection related metadata includes active Node list and cluster connection permission control policy. Based on the metadata, RDMA Service know to whether it is permitted to and and how it sets up virtual TCP connections. 
\end{enumerate}

In order for RDMA Connection Manager to multiplex TCP connection over one single RDMA Connection, TSoR introduce a concept of RDMA Channel as Figure 5. RDMA Channel is a logic virtual data connection between 2 Cluster Nodes. One RDMA Chanel has 2 data ring buffers (i.e. Read buffer and Write buffer) in each side of the connection. The Read Buffer on one side will connect to the Write Buffer of the other side. The ring buffer is pined as Memory Range (MR) of RDMA Connection so that the data from local Write Buffer could be write by RDMA NIC to remote peer's Read Buffer. One RDMA Connection has one RDMA Control Channel and multiple RDMA Data Channels. The RDMA Control Channel is used for the control message transmit between the Nodes; and the RDMA Data Channel is used for TCP data transmit. One TCP connection will be mapped to one RDMA Data Channel. 

RDMA supports different types data operations such as Send, Receive, RDMA Write, etc. We choose RDMA Write With Immediate for TCP traffic transfer. RDMA Write With Immediate operation could copy a user space buffer data to remote machine application buffer as a common Write operation. And when the copy is done, it will also wake up remote RDMA service with another TSoR defined 32 bits immediate data. The 32 bites immediate data will help TSoR multiplex TCP socket connections over one RDMA Connection. The design choice can achieve lower latency with compromising of the system throughput.

RDMA Service's main thread is a polling thread and will keep polling the event from underlying RDMA Connections and the queue pairs of TSoR client. It won't call any host OS system call in the active processing so that it could get low latency and high throughput. 
 
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/RDMAChannel.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 
 
\subsection{TSoR Client}

\zhao{need new subsection title}

By default, Quark runtime will simulate the TCP system calls based on host Linux system call interface. In TSoR environment, TSoR Client will take over the TCP system call requests and simulate them with underlying RDMA connection based on the service provided by RDMA Client Manager.

TSoR Client communicates with the RDMA Client Manager through the message queue pair and exchange TCP traffic data through the Shared Buffers described in section 4.1. There are 2 types of TCP requests:
\begin{itemize}
\item \textbf{Control requests}: e.g. connect, listen, accept, close. When TSoR Client gets such requests, it will use the message queue pair to ask the RDMA Service to allocate the ring buffers and setup/tire down the TCP connection's related RDMA Channel;
\item \textbf{Data requests}: e.g. Send, Recv, Read, Write. When TSoR Client gets such request, it will write to TSoR write buffer or read from TSoR read buffer of Shared Buffers and notify the RDMA Service.
\end{itemize}
 
TSoR Client is integrated by both Quark pod and TSoR Gateway. It also handles the TSoR Gateway external TCP connection request just like user applications running in Quark pod.

\subsection{TSoR Gateway}

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TSoRGateway.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 User application running in Quark Pod of TSoR Cluster needs to access to external service (Egress) and TSoR cluster also needs to allow external service to access internal Quark Pod (Ingress) with TCP protocol. As the TSoR Cluster's internal network traffic is over RDMA, a TSoR Gateways is needed for the protocol transformation between TCP and RDMA protocol. 
 
 Figure 8 show s the TSoR Gateway architecture. The TSoR Gateway has following main components:
 
\begin{itemize}
\item \textbf{TSoR Client}: As Quark Pod, there is one TSoR Client running inside TSoR Gateway which handle the communication with RDMA Service. 
\item \textbf{Gateway Control Plane Agent}: TSoR Agent needs to ask the network policy and Pod address information from cluster Control Plane.
\item \textbf{Ingress TCP layer}: It will accept external TCP connection and forward the TCP traffic to the target Quark Pod through RDMA. It takes a DNAT role in TCP/IP protocol stack.
\item \textbf{Egress TCP layer}: It will forward the internal TCP connection to external. It takes the SNAT role in TCP/IP protocol stack.
\end{itemize}

The TSoR Gateway is running in a common host OS process instead of in Quark container. It could save the virtualization cost and improve the performance.

% \subsection{Technical Decisions }
% To transfer TCP traffic using RDMA network, TSoR has following technical choices:
 
%  \textbf{RDMA operation choice}: RDMA supports different types operations such as Send, Receive, RDMA Write, etc. We choose RDMA Write With Immediate for TCP traffic transfer. RDMA Write With Immediate operation could copy a user space buffer data to remote machine application buffer as Write operation. And when the copy is done, it will also wake up remote RDMA service with another TSoR defined 32 bits immediate data. The 32 bites immediate data will help TSoR multiplex TCP socket connections over one RDMA QP connection. The choice can achieve lower latency with compromising of the system throughput.




==> design_original.tex <==
\section{Design and Implementation}
TSoR has the following design goals:
\begin{itemize}
\item {\bf Performance improvement for TCP traffic}: TSoR is designed to leverage RDMA NIC to transmit TCP traffic. It should have increased throughput and decreased latency.
\item {\bf Transparency to the application programmer}: TSoR is designed to significantly improve performance without requiring modifications to applications or containerized image.
\item {\bf Multi-tenant isolation support}: TSoR is designed to support isolating network traffic between different tenants.
\item {\bf Fast container start up and tear down}: TSoR is designed to support serverless container computing which means container will be started and stopped frequently, fast container start up and tear down is a must.
\item {\bf Kubernetes network model compatibility}: TSoR is designed to be fully compatible with Kubernetes network model. There should be minimal effort to set up TSoR for existing Kubernetes cluster so that it can be used in existing Kubernetes ecosystem.
\end{itemize}
In this section, we show how we achieve these goals in TSoR. We describe the infrastructure requirement for this architecture, and we detail interface and design of the control plane and data plane of TSoR. Finally, we describe our implementation of TSoR based on secure container runtime Quark.

\subsection{Architecture Overview}

TSoR targets cluster which has RDMA network support. Figure 2 shows the overall architecture. TSoR control plane assign container IP, get nodes and containers information from Kubernetes API Server. TSoR data plane use information from control plane to set up RDMA connections between cluster nodes, established TCP connections and transfer TCP traffic using RDMA IB verbs. Traffic inside cluster using TSoR will leverage RDMA, TSoR gateways are introduced to transform traffic between TCP and RDMA when communicating with outside cluster entities.
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TSoRArchPlanes.png}
 \caption{TSoR Architecture}
%  \label{fig::arch}
 \end{figure}
\subsection{TSoR Interface}
There're 2 categories of interface when using TSoR:

{\bf 1. Application Programming Interface}

Applications still use normal POSIX socket API[] for TCP related operations. As socket API calls interception happens in Quark's system call virtualization layer, that means it doesn't need any code modification or rebuilding of application, even existing container image can use TSoR directly which provides transparency to application programmers.

{\bf 2. Kubernetes related interface}
TSoR supports Kubernetes networking model including container IP address assignment, service, DNS based service discovery and intra-cluster load balance so that TSoR can be applied to existing Kubernetes cluster with minimal effort.

\subsection{TSoR Control Plane}
TSoR control plane is responsible for container IP assignment, supporting Kubernets network model and talking to Kubernets API server to watch node and container information.

\textbf{Container IP address assignment}: TSoR supports multi-tenant container IP address assignment. Different tenants could share the same CIDR. The assigned address could be expressed as a tuple <Tenant ID, IP Address>.  Each container has its tenant id when start up by TSoR. When TSoR allocates IP address for a new container, it will assign the container’s Tenant ID first, then allocate the available IP address based on that. Currently TSoR use fixed CIDR for all the tenants on one cluster node. The reason of this design is to eliminate IP Address route propagation latency for the frequent container start up and tear down. Because each cluster node has a fixed subnet CIDR for all tenants, RDMA service could create CIDR to neighbor cluster node mapping. The mapping will only be updated when there is node added and deleted. When RDMA gets a TCP connection request, it can simply look up the mapping based on  the target IP address’s CIDR to get the remote cluster node no matter which tenant the container belongs to.
\subsection{TSoR Data Plane}
The main goal of TSoR is to provide a faster container network by transferring TCP traffic over the RDMA network. TSoR will intercept TCP socket system calls, create RDMA connection between TCP client and TCP server and transfer TCP data through the RDMA connection. Figure 3 shows an example data transfer process using TSoR. In this example, there are 2 Quark containers, i.e. Client application and Server application, are running on 2 bare-metal machines, i.e. Node1, Node2. There are RDMA networks available between them.  In the example scenario, the client application will use a TCP connection to send data to the server application. The underlying data sending process is as below.

\textbf{1. Sys\_send system call}: Client Application call system call sys\_send to ask OS kernel to send data in a user space buffer to Server Application;

\textbf{2. Memory copy from user space to OS kernel}: The Quark OS kernel takes over control through the sys\_send system call and copy the data from user space to the Quark kernel socket send buffer;

\textbf{3. RDMA data transfer}: As there is an RDMA network between the 2 nodes, the client Quark OS kernel will use RDMA IB verbs to write the data to the Server application’s Quark kernel socket recv buffer;

\textbf{4. Memory copy from OS kernel to user space}: After the data is written to the Server application Quark Kernel recv buffer, the server Quark kernel will copy it to the server application’s application recv buffer.

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/data_path.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 
As Figure3 shows, the interception of TCP socket releated calls happens at Quark System Call Virtualization layer so it's totally transparent to application.

\subsection{TSoR Gateway}
Network traffic will be transmitted using RDMA network inside cluster using TSoR. To make services in cluster available to external world or access services outside of cluster, TSoR gateways are designed and implemented to do transformation between TCP traffic and RDMA traffic. 
% Both QuarkIngress and QuarkEgress gateway have a rdma\_srv\_cli talking to RDMA Service while using TCP socket to talk to outside cluster world.

% \subsection{Serverless Container Network}
% The goal of TSoR is to provide a container network which can transfer TCP traffic over the RDMA network. It will intercept TCP socket system calls, create RDMA connection between TCP client and TCP server and transfer the TCP data through the RDMA connection. An example data transfer process is below. In this example, there are 2 Quark containers, i.e. Client application and Server application, are running on 2 bar-metal machines, i.e. Node1, Node2. There are RDMA networks available between them.  In the example scenario, the client application will use a TCP connection to send data to the server application. The underlying data sending process is as below.

% \textbf{1. Sys\_send system call}: Client Application call system call sys\_send to ask OS kernel to send data in a user space buffer to Server Application;

% \textbf{2. Memory copy from user space to OS kernel}: The Quark OS kernel takes over control through the sys\_send system call and copy the data from user space to the Quark kernel socket send buffer;

% \textbf{3. RDMA data transfer}: As there is an RDMA network between the 2 nodes, the client Quark OS kernel will use RDMA IB verbs to write the data to the Server application’s Quark kernel socket recv buffer;

% \textbf{4. Memory copy from OS kernel to user space}: After the data is written to the Server application Quark Kernel recv buffer, the server Quark kernel will copy it to the server application’s application recv buffer.

% \begin{figure}[tbp]
%      \centering
%  \includegraphics[width=\linewidth]{graphs/charts/data_path.png}
%  \caption{}
% %  \label{fig::arch}
%  \end{figure}
 
 The RDMA Verbs supports Reliable Connection (RC) , i.e. RC Queue Pair (QP). The RC QP handles TCP protocol’s functionality like congestion control and loss recovery. TSoR relies on RC QP and doesn’t need to worry about the reliable connection work. But it still has to handle the following data plane challenges.
 
 \textbf{TCP connection creation latency}: The RDMA RC QP creation needs another communication channel, e.g. TCP, to help exchange QP metadata. We measured the latency of creating such RC QP based on TCP connection and found the latency is about 5000 microsecond while a normal TCP connection creating latency is about 350 microsecond.
 
\textbf{RDMA QP scalability}: In the design of SMC[] and DirectSocket[], one TCP connection has one underlying RDMA QP. In the typical cluster environment, the microservices running on one bar-metal machine might need 1 million TCP connections. If we are using such 1:1 mapping, it is hard for RDMA NIC to support so many QPs and with  the QP count increases, the RDMA NIC performance will decrease.

TSoR also needs to support container network virtualization functions. Besides Kubernetes network mode required functions such as service discovery, QoS, TSoR are facing more serverless challenges as below.

\textbf{Serverless container IP address assignment}: The serverless container deployment density might be much higher than single tenant Kubernates environment. For example, RunD[] supports running 2500 containers. Furthermore, the serviceless container needs to frequently start up and tear down. TSoR needs to support such scalability for the multitenant container IP allocation. And the new assigned IP address route information should be propagated efficiently in the cluster;

\textbf{Data Ingress and egress}: In TSoR support cluster, the intra Pod connection will be based on RDMA. But its external connection should still go through TCP/IP. Special ingress/egress gateways are needed to switch data between TCP and RDMA.

\textbf{Network QoS}: TSoR is a multi-tenant container network provider. It needs support control of the network bandwidth and priority of different tenants.

\subsection{Design principle and Architecture}
In the TSoR enabled Quark cluster, there are multiple cluster nodes with multiple Quark containers running on that. Between containers, multiple TCP streams are created to transfer intra- or inter- cluster node data traffic.

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/key_concept.png}
 \caption{Overview}
%  \label{fig::arch}
 \end{figure}

To address the design challenges, TSoR takes the following design concepts.

\textbf{Multiplex TCP streams over RDMA RC QP}: Because of the RDMA NIC QP count limitation, we multiplex TCP over RDMA QPs. When there is TCP data ready for transfer between Quark containers, TSoR will choose one existing RDMA connection to transfer the data. One single RDMA connection will transfer multiple TCP streams data. This is designed to mitigate the RDMA NIC scalability issue.

\textbf{Pre-created RDMA QP when cluster node bootup}: The TSoR will create a RDMA connection mesh between all cluster nodes. When one cluster node bootup, it will look for all running cluster nodes and create RDMA connections with them. This design will decrease the TCP connection creation latency.

\textbf{Per node RDMA service}: There is one single RDMA service per cluster node. On one hand, the RDMA service will manage all the RDMA QPs of the cluster node; on the other hand all the TCP streams of the node will be aggregated in the RDMA service. The RDMA service will enforce the TCP streams network policy, QoS in addition to Kubernetes container network mode requirement.

In this section, we describe the TSoR architecture and design principle as figure 1 shows. TSoR’s major components are as below.

\textbf{rdma\_srv}: RDMA service (rdma\_srv) is a daemon process that executes separately from containers. Each cluster node sets up one single rdma\_srv. rdma\_srv is to handle the RDMA connections between all cluster nodes.

\textbf{rdma\_agent}: rdma\_srv sets up one RDMA agent (rdm\_agent) for each container. rdma\_agent is to push/pop requests which are fed to SubmitQueues /CompleteQueues between rdma\_srv\_cli and rdma\_srv. rdma\_agent is to create one channel to exchange data between containers and rdma\_srv.

\textbf{rdma\_srv\_cli}: Each container will set up a RDMA service client (rdma\_srv\_cli). All data traffic goes through the connection between rdma\_srv and rdma\_srv\_cli. rdma\_srv\_cli is to push/pop requests which are fed to SubmitQueues /CompleteQueues between rdma\_srv\_cli and rdma\_srv.

\textbf{rdma\_channel}: Each TCP connection has one rdma channel to send/recv data between rdma\_srv\_cli and rdma\_srv. Each channel is based on shared memory data structures (client\_share\_region described later) including Queues and IO buffers.

\textbf{rdma\_connection}:  Cluster nodes set up the RDMA connection (rdma\_connection) between each other. rdma\_connection is multiplexed for all containers and the TCP connections between the same pair of nodes.

\textbf{client share region}: ClientShareRegion is for the communication between rdma\_srv\_cli and rdma\_agent. cq/sq are shared memory queues to exchange requests. iobuf is a buffer mapped to a socket buffer where the system calls write/read data to/from.

\subsection{TCP socket over RDMA}
TSoR is using RDMA IB verbs to transfer TCP stream data. RDMA IB verbs can copy user space application data buffers between cluster nodes. RDMA requires the data buffer be pre-register to the RDMA NIC before transfer data for it. TCP kernel buffer design and IB verbs choice will impact data transfer performance and memory consumption. TSoR takes following design for the TCP data transfer:

\textbf{2 Ring buffers for each TCP socket}: For each TCP socket, TSoR creates 2 fixed size ring buffers, i.e. read buffer and write buffer, when TCP connections are created for the socket. The Ring buffer memory is shared between the Quark container and RDMA service and  is registered in RDMA. RDMA\_srv uses IB verbs to copy ring buffer data between cluster nodes and synchronize the ring buffer head/tail pointer.

\textbf{RDMA write\_immdiate verb}: There are multiple data copy IB verbs. TSoR chose write\_immdiate verb for socket buffer data copy. write\_immdiate sends another 32 bites immediate data together with data copy and wake up remote RDMA service when copy finishes. The 32 bites immediate data will indicate the RDMA channel id. The choice can achieve better latency but it might hurt the system throughput.

\textbf{TCP connecting process}
TSoR leverage RDMA to establish TCP connection which can help reduce latency.TCP connection starts from client application calling connect, following section illustrates TCP connection process using TSoR.

\textbf{1.Push Connect Request to submission queue}:rdma\_srv\_cli enqueues one connect request to submission queue between rdma\_srv\_cli and rdma\_srv.

\textbf{2.Client side rdma\_srv handle Connect Request}:rdma\_srv parses Connect Request, calculates the peer node based on destination container IP in Connect Request, creates rdma\_channel, constructs a connection request and sends it over to peer node via control channel using IB Verb: RDMA Write Immediate.

\textbf{3.Server side rdma\_srv handle connection request}:rdma\_srv parse connection request, verify whether there's a container listening on destination {TenantId, IP, port}.
If so, rdma\_srv creates rdma\_channel, enqueue an accept request to Completion Queue of the container which is listening on destination tuple {TenantId, IP, port}. At the same time, rdma\_srv construct connection response request and send it back to client node via RDMA.

\textbf{4.Client side rdma\_srv handle connection response}: Client side rdma\_srv parse connection response,save peer rdma\_channel id, construct and enqueue Connect Response to client container

\textbf{5.Client side container handle connection response}: Client side container parse connection response, notify application that connection is established and data can be sent. 
\textbf{Data transfer process}


\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/write_flow.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 
 Figure shows TSoR’s TCP data transfer process which has the following steps.
 
\textbf{1. Ringbuffer Produce}: By this step, SysWrite plays as the producer for the socket buffer and copies data from the application to the writeBuf.

\textbf{2. Push Write\_Request to the submit queue}: rdma\_srv\_cli enqueues one write request into the submit queue between rdma\_srv\_cli and rdma\_srv.

\textbf{3. RDMA data copy to remote peer}: RDMA\_srv copy the data from local write buffer to remote read buffer with write\_immediate IB verb.

\textbf{4. Rdma\_srv processes the received write\_immediate}: The remote rdma\_srv will get notification from RDMA NIC when the data copy is finished. Then RDMA\_srv will notify rdma\_srv\_cli there is data ready for reading in the read buffer by enqueue request in the completion queue between RDMA\_srv and rdma\_srv\_cli.

\textbf{5.  SysRead consumes the read buffer}: SysRead consumes the read buffer and will copy the data from kernel read buffer to application buffer.

\subsection{RDMA based container network}
The TSoR meets Kubernetes container network requirements and extends its function to support multi-tenant serverless network isolation, scalability etc. As figure\#3, TSoR RDMA service has a control plane connection with Kubernetes APIServer. From the APIServer, RDMA service could get cluster information such as cluster active node ip address list, Kubernetes service endpoints and cluster IPs. And based on such data, RDMA will do the following control  plane work.

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/rdma_cluster.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}

\textbf{RDMA QP creation}: When RDMA service starts up, it will firstly retrieve the active cluster node list from APIServer. And then it will create RDMA connections to all the remote cluster nodes. The RDMA connections will be used for later TCP connection establishment and TCP data transfer;

% \textbf{Container IP address assignment}: TSoR supports multi-tenant container IP address assignment. Different tenants could share the same subnet CIDR. So the assigned address could be expressed as a tube <Tenant ID, IP Address>.  Each Quark container has its tenant id when start up by TSoR. When TSoR allocates IP address for a new container, it will firstly get the container’s Tenant ID and then allocate the free IP address based on that. So far, TSoR used fixed subnet CIDR for all the tenants on one cluster node. The reason of this design is to save IP Address route propagate latency for the frequent container start up and tear down. Because each cluster node has a fixed subnet CIDR for all tenants, RDMA service could create a CIDR to neighbor cluster node mapping. The mapping will only be updated when there is node bootup and shutdown. When RDMA gets a TCP connection request, it can simply look up the map based on  the target IP address’s CIDR to get the remote cluster node no matter which tenant the container belongs to.
% \subsection{Ingress/Egress Gateway}
% Network traffic will be transmitted using RDMA inside cluster using TSoR. To make services in cluster available to external world or access services outside of Cluster, QuarkIngress and QuarkEgress gateways are designed and implemented to do transformation between TCP traffic and RDMA traffic. Both QuarkIngress and QuarkEgress gateway have a rdma\_srv\_cli talking to RDMA Service while using TCP socket to talk to outside cluster world.

\textbf{QuarkIngress Gateway}

QuarkIngress Gateway is responsible for transforming TCP traffic from outside to RDMA traffic inside cluster using TSoR.
A Kubenetes custom resource definition called RDMAIngress is introduced to set up mapping between external port and internal service. QuarkIngress gateway will listen on the external port for incoming TCP connection request and traffic. On the other side QuarkIngress uses rdma\_srv\_cli to talk to RDMA service for TCP traffic and RDMA transformation. 

\textbf{QuarkEgress Gateway}
QuarkEgress Gateway is responsible for transforming RDMA traffic inside cluster using TSoR to outside cluster service.
RDMA Service will forward request to QuarkEgress gateway if traffic destination is not for containers inside cluster. QuarkEgress then uses TCP socket to connect to outside cluster service.

% \subsection{Zero memory copy TCP socket extension}
% TSoR provides a RDMA based TCP stack which has better performance than TCP/IP protocol stack. But its performance is still lower than native RDMA applications. One performance overhead is from BSD socket memory copy between user space and OS kernel. So the TSoR proposes and implements a zero memory design for TCP socket in Quark. The design has 2 parts:

% \textbf{Memory mappable TCP socket}: As we discussed in 3.3, TSoR creates 2 fixed size ring buffers (one is read buffer and the other is write buffer) for each TCP socket. The buffers are memory page aligned. TSoR extends sys\_mmap to enable it for TSoR TCP sockets. So the user application can memory map the 2 buffers to user space and then it can use it as user application buffer to avoid extra memory copy.

% \begin{figure}[tbp]
%      \centering
%  \includegraphics[width=\linewidth]{graphs/charts/zero_copy.png}
%  \caption{}
% %  \label{fig::arch}
%  \end{figure}
 
% \textbf{2 more system calls to handle ring buffer head/tail pointers}: The 2 socket kernel buffers are managed as ring buffers with head and tail pointers. TSoR adds 2 system calls to enable user application get/set the head/tail pointer. The 2 system calls signatures are as below.
% \[
% int~sys\_socket\_consume(int: fd, int: count, *iovec: addr, int: flags)
% \]

% This is for the read buffer. It tells Quark Kernel that the $count$ bytes of the read buffer has been consumed by the user application and is Ok to overwrite more data from remote peer. The iovec is an out parameter and returns the iovec array of available data ranges in the read buffer.
% \[
% int~sys\_socket\_produce(int: fd, int: count, *iovec: addr, int: flags)
% \]
% It is for the write buffer. It tells Quark Kernel that the count bytes of the write buffer has been produced by the user application and is ready to send to the remote peer. The iovec is an out parameter and returns the iovec array of free space range.





==> design_zcxy.tex <==


\newpage
\section{Overview}

\textbf{Design Goals / Motivation}:

1) High-performance RDMA network for container

2) Transparency: Compatible with POSIX Socket and Container Runtime

3) Integration with K8S / Kubernetes network model compatibility:

-Control Plane: overlay network

-Multi-tenant isolation support

-Fast container start up and tear down (efficient routing):


\noindent\textbf{Sections}:

1) App POSIX Interface and Lightweight VM

- Quark (syscall) virtualization layer

- POSIX  

2) Data Path: RDMA\_Service

-control: QP connection setup

-control: socket connection 

-data: Data Transfer

3) Control Plane: K8S , Ingress/Egress Gateway

\section{CNI/Runtime: App POSIX Interface}
- Quark (syscall) virtualization layer
- POSIX 

\section{Control Plane}
\subsection{Meta Data}

\section{RDMA\_Service}
\subsection{Concept}
\subsection{Node-to-Node QP}
-Challenge

-Solution
\subsection{Socket Connection}
\subsection{Data Transfer}

\section{Gateway}


==> designandimplementation.tex <==
\section{Design and Implementation}
This section illustrates TSoR design and implementation. We will present the challenges first and how we address those along with reasoning for different technical decisions. After that, we will introduce TSoR high level module design and the implementation details.  
\subsection{Challenges and Technical Decisions}
To transfer TCP traffic using RDMA network, TSoR has following technical choices and chanllenges:

 \textbf{RDMA Queue Pair choice}: RDMA supports different types of Queue Pair. We choose Reliable Connection(RC) Queue Pair(QP) for TCP socket connection. The RC QP handles TCP protocol’s functionality such as congestion control and loss recovery. TSoR relies on RC QP and doesn’t need to worry about the reliable connection work. But it still has to handle the following data plane challenges.
 
 \textbf{RDMA operation choice}: RDMA supports different types operations such as Send, Recieve, RDMA Write, etc. We choose RDMA Write With Immediate for TCP traffic transfer. RDMA Write With Immediate sends another 32 bits immediate data together with data copy and wake up remote RDMA service when copy finishes. The 32 bites immediate data will help TSoR multiplex TCP socket connections over one RDMA QP connection. The choice can achieve better latency but it might hurt the system throughput.
 
 \textbf{RDMA QP scalability chanllenge}: In the design of SMC[] and DirectSocket[], one TCP connection has one underlying RDMA QP. In a typical cluster environment, the microservices running on one bar-metal machine might need 1 million TCP connections. If we are using 1:1 mapping between TCP socket and QP, it is hard for RDMA NIC to support so many QPs and with  the QP count increases, the RDMA NIC performance will decrease[]. We address this challenge by multiplexing TCP streams over RDMA RC QP. Two cluster nodes will set up only one RC QP for all TCP socket connection between them. 
 
 \textbf{RC QP connection establishment latency}: The RDMA RC QP connection establishment needs another communication channel, e.g. TCP, to help exchange QP metadata. We measured the latency of creating such RC QP based on TCP connection and found the latency is about 5000 microsecond. To address this issue, TSoR establish RC QP connections when nodes are added into cluster. TCP socket connections will use this pre established QP connection.

To support Kubernetes network model including IP assignment, service discovery and QoS, TSoR are facing following challenges:

\textbf{Serverless container IP address assignment}: The serverless container deployment density might be much higher than single tenant Kubernetes environment. For example, RunD[] supports running 2500 containers on each node. Furthermore, container in serverless environment needs to frequently start up and tear down. TSoR needs to support such scalability for the multi-tenant container IP allocation while the routing should still be efficient. At the same time, TSoR need support traffic isolation between different tenants. To address these chanllenges, TSoR allows different tenants to share same CIDR. The assigned address could be expressed as a tuple <Tenant ID, IP Address>.  Each container has its tenant id when start up by TSoR. When TSoR allocates IP address for a new container, it will assign the container’s Tenant ID first, then allocate the available IP address based on that. Currently TSoR use fixed CIDR for all the tenants on one cluster node. The reason of this design is to eliminate IP Address route propagation latency for the frequent container start up and tear down. Because each cluster node has a fixed subnet CIDR for all tenants, RDMA service could create CIDR to neighbor cluster node mapping. The mapping will only be updated when there is node added and deleted. When RDMA gets a TCP connection request, it can simply look up the mapping based on  the target IP address’s CIDR to get the remote cluster node no matter which tenant the container belongs to.


\textbf{TSoR Gateway}: Network traffic will be transmitted using RDMA network inside cluster using TSoR. To make services in cluster available to external world or access services outside of cluster, TSoR gateways needs do transformation between TCP traffic and RDMA traffic in addition to standard Kubernetes gateway functionalities.

% In TSoR support cluster, the intra Pod connection will be based on RDMA. But its external connection should still go through TCP/IP. Special ingress/egress gateways are needed to switch data between TCP and RDMA.


\textbf{Network QoS}: TSoR is a multi-tenant container network provider. It needs support control of the network bandwidth and priority of different tenants. TSoR introduces a separate service called RDMA service to serve all containers on one cluster node instead of a component residing in container to address this requirement.

\subsection{High level module design}
As Figure 4 shows, TSoR introduces following modules:

\textbf{RDMA Connection Manager(CM)}: RDMA CM is responsible for talking to Kubernetes API server to watch node/pod information and server them to RDMA Service. It is also in charge of container IP address assignment. Currently RDMA CM is a separate process running in each cluster node.

\textbf{RDMA Service}: RDMA Service is a core module of TSoR and a daemon service running in each cluster node. RDMA service is the only module to talk to RDMA NIC and serve all containers (including TSoR Ingress and Egress mentioned below) running on current cluster node. It is responsible for following tasks:
\begin{itemize}
\item {\bf Manage RDMA Queue Pairs}: Using nodes information from RDMA CM to set up RDMA QP connection between clust nodes when nodes join cluster.
\item {\bf Serve container requests for all TCP socket related operations}: Using container information from RDMA CM to establish TCP socket connection, transfer TCP traffic and server other TCP socket related operations using RDMA network.
\item {\bf Traffic routing and isolation between different tenants}: Using container CIDR and cluster node mapping to do traffic routing and using tenant id to enforce traffic isolation.
\item {\bf Quality of Service enforcement}: ??.
\item {\bf Support Kubernetes service}: RDMA Service supports Kubernetes service to be compatible with existing Kubernetes deployment paradigm. It also support load balancing between container instances behind service.
\end{itemize}

\textbf{QuarkIngress Gateway}

QuarkIngress Gateway is responsible for transforming TCP traffic from outside to RDMA traffic inside cluster using TSoR.
A Kubenetes custom resource definition called RDMAIngress is introduced to set up mapping between external port and internal service. QuarkIngress gateway will listen on the external port for incoming TCP connection request and traffic. On the other side QuarkIngress uses rdma\_srv\_cli to talk to RDMA service for TCP traffic and RDMA transformation. 

\textbf{QuarkEgress Gateway}
QuarkEgress Gateway is responsible for transforming RDMA traffic inside cluster using TSoR to outside cluster service.
RDMA Service will forward request to QuarkEgress gateway if traffic destination is not for containers inside cluster. QuarkEgress then uses TCP socket to connect to outside cluster service.

\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TSoRArchModule.png}
 \caption{TSoR Modules}
%  \label{fig::arch}
 \end{figure}

Different communication mechanisms are used between aforementioned TSoR modules:
\begin{itemize}
\item {\bf Between RDMA CM and RDMA Service}: RDMA Service connects to RDMA CM using gRPC.
\item {\bf Between RDMA Service and Containers}: Quark containers uses Unix Domain Socket to exchange memory information before creating a shared memory region. After that, two queues, Submit Queue and Completion Queue, in the shared memory will be used to send request and response between RDMA Service and Containers.
\item {\bf Between Gateways and RDMA Service}: TSoR gateways uses same aforementioned mechanism as containers when talking to RDMA service. They use vanilla TCP socket APIs when talking to external world.
\end{itemize}

\subsection{RDMA Service components and concepts}
In this section, we describe RDMA service major components and concepts. They will be used to illustrate workflows in coming sections.

\textbf{rdma\_srv}: rdma\_srv is a global component inside RDMA service, it maintains global entities such as rdma\_agents, rdma\_connections and rdma\_channels.

\textbf{rdma\_srv\_cli}: Each container including TSoR Ingress and Egress Gateway will set up a RDMA service client (rdma\_srv\_cli). Quark containers and gateways will delegate all TCP socket related operations to rdma\_srv\_cli which then talks to RDMA service via Submit Queues and Complete Queues residing in shared memory between rdma\_srv\_cli and RDMA Service.


\textbf{rdma\_agent}: RDMA Service sets up one RDMA agent (rdm\_agent) for each container and TSoR gateway. rdma\_agent is to pop/push requests which are fed to Submit Queues /Complete Queues between rdma\_srv\_cli and RDMA Service.

\textbf{rdma\_channel}: One rdma\_channel will be created for each TCP socket connection. rdma\_channel is responsible managing ring buffer which is shared between TCP socket and rdma\_channel to prepare data before leveraging RDMA network to send.

\textbf{rdma\_connection}: RDMA Service on each cluster node will set up the RDMA connection (rdma\_connection) between each other node. rdma\_connection is multiplexed for rdma\_channel on current node to send and receive RDMA traffic.

\textbf{rdma\_control\_channel}: One rdma\_control\_channel is created for each rdma\_connection. rdma\_control\_channel is used to exchange rdma\_channel establishment information and other metadata such as remote receive request count.

\textbf{client share region}: ClientShareRegion is a shared memory region between rdma\_srv\_cli and rdma\_agent. cq/sq are lock free shared memory queues to exchange request/response between rdma\_srv\_cli and rdma\_agent. iobuf is a buffer mapped to a socket buffer where the system calls write/read data to/from.
\subsection{RDMA Queue Pair Connection Establishment}
When RDMA service starts up after node joins cluster, it will use following steps to set up RDMA QP Connection:
\begin{enumerate}
\item Start TCP server to listen on a known port to wait for RDMA service on other nodes to connect
\item Retrieve active cluster node list from RDMA CM. Each node entity will has a timestamp which shows it's time to join the cluster.
\item Compare other node timestamp with timestamp on current node. Connect to RDMA service on nodes which timestamp is earlier than current node using TCP socket API.
\item Create rdma\_connection and rdma\_control\_channel using TCP socket connection to exchange RDMA RC QP and rdma\_control\_channel metadata.
\end{enumerate}

\subsection{TCP socket connection establishment}
TCP uses a three-way handshake to establish a reliable connection which can take time around 300 microseconds. RDMA network has much lower latency, TSoR uses RDMA network(rdma\_control\_channel is used under the hood)to exchange metadata when establishing TCP socket connection following below steps(?? sequential diagram):
\begin{enumerate}
\item {\bf Push Connect Request to submission queue}:rdma\_srv\_cli enqueues one connect request to submission queue between rdma\_srv\_cli and RDMA Service.

\item {\bf Client side rdma\_srv handle Connect Request}:rdma\_srv parses Connect Request, calculates the peer node based on destination container IP in Connect Request, creates rdma\_channel, constructs a connection request and sends it over to peer node via control channel using IB Verb: RDMA Write Immediate.

\item {\bf Server side rdma\_srv handle connection request}:rdma\_srv parse connection request, verify whether there's a container listening on destination {TenantId, IP, port}.
If so, rdma\_srv creates rdma\_channel, enqueue an accept request to Completion Queue of the container which is listening on destination tuple {TenantId, IP, port}. At the same time, rdma\_srv construct connection response request and send it back to client node via RDMA.

\item {\bf Client side rdma\_srv handle connection response}: Client side rdma\_srv parse connection response,save peer rdma\_channel id, construct and enqueue Connect Response to client container

\item {\bf Client side container handle connection response}: Client side container parse connection response, notify application that connection is established and data can be sent. 
\end{enumerate}

\subsection{TCP socket data transfer process}
TSoR is using RDMA IB verbs to transfer TCP stream data. RDMA IB verbs can copy user space application data buffers between cluster nodes. RDMA requires the buffer memory to be pre-registered to the RDMA NIC before data transfer. TCP kernel buffer design impact data transfer performance and memory consumption. For each TCP socket, TSoR creates 2 fixed size ring buffers, i.e. read buffer and write buffer, when TCP connections are created for the socket. The Ring buffer memory is shared between the Quark container and RDMA service and  is registered in RDMA. RDMA service uses IB verbs to copy ring buffer data between cluster nodes and synchronize the ring buffer head/tail pointer with Quark container.

% \textbf{TCP connecting process}
% TSoR leverage RDMA to establish TCP connection which can help reduce latency.TCP connection starts from client application calling connect, following section illustrates TCP connection process using TSoR.
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/write_flow.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 
Figure shows TSoR’s TCP data transfer process which has the following steps.
\begin{enumerate}
\item {\bf Ringbuffer Produce}: By this step, SysWrite plays as the producer for the socket buffer and copies data from the application to the writeBuf.

\item {\bf Push Write\_Request to the submit queue}: rdma\_srv\_cli enqueues one write request into the submit queue between rdma\_srv\_cli and rdma\_srv.

\item {\bf RDMA data copy to remote peer}: RDMA\_srv copy the data from local write buffer to remote read buffer with write\_immediate IB verb.

\item {\bf Rdma\_srv processes the received write\_immediate}: The remote rdma\_srv will get notification from RDMA NIC when the data copy is finished. Then RDMA\_srv will notify rdma\_srv\_cli there is data ready for reading in the read buffer by enqueue request in the completion queue between RDMA\_srv and rdma\_srv\_cli.

\item {\bf SysRead consumes the read buffer}: SysRead consumes the read buffer and will copy the data from kernel read buffer to application buffer.
\end{enumerate}
\subsection{Implementation}
Except RDMA Connection Manager, all other modules (RDMA Service, Ingress, Egress and changes in Quark container runtime) of TSoR are written in Rust language to achieve efficiency and safety. The rust code is around 30k line. RDMA Connection Manager is using golang mainly together with Rust building the service client. Total lines are around 10k. 


% \subsection{RDMA based container network}
% The TSoR meets Kubernetes container network requirements and extends its function to support multi-tenant serverless network isolation, scalability etc. As figure\#3, TSoR RDMA service has a control plane connection with Kubernetes APIServer. From the APIServer, RDMA service could get cluster information such as cluster active node ip address list, Kubernetes service endpoints and cluster IPs. And based on such data, RDMA will do the following control  plane work.

% \begin{figure}[tbp]
%      \centering
%  \includegraphics[width=\linewidth]{graphs/charts/rdma_cluster.png}
%  \caption{}
% %  \label{fig::arch}
%  \end{figure}


% \textbf{Container IP address assignment}: TSoR supports multi-tenant container IP address assignment. Different tenants could share the same subnet CIDR. So the assigned address could be expressed as a tube <Tenant ID, IP Address>.  Each Quark container has its tenant id when start up by TSoR. When TSoR allocates IP address for a new container, it will firstly get the container’s Tenant ID and then allocate the free IP address based on that. So far, TSoR used fixed subnet CIDR for all the tenants on one cluster node. The reason of this design is to save IP Address route propagate latency for the frequent container start up and tear down. Because each cluster node has a fixed subnet CIDR for all tenants, RDMA service could create a CIDR to neighbor cluster node mapping. The mapping will only be updated when there is node bootup and shutdown. When RDMA gets a TCP connection request, it can simply look up the map based on  the target IP address’s CIDR to get the remote cluster node no matter which tenant the container belongs to.
% \subsection{Ingress/Egress Gateway}
% Network traffic will be transmitted using RDMA inside cluster using TSoR. To make services in cluster available to external world or access services outside of Cluster, QuarkIngress and QuarkEgress gateways are designed and implemented to do transformation between TCP traffic and RDMA traffic. Both QuarkIngress and QuarkEgress gateway have a rdma\_srv\_cli talking to RDMA Service while using TCP socket to talk to outside cluster world.



% \subsection{Zero memory copy TCP socket extension}
% TSoR provides a RDMA based TCP stack which has better performance than TCP/IP protocol stack. But its performance is still lower than native RDMA applications. One performance overhead is from BSD socket memory copy between user space and OS kernel. So the TSoR proposes and implements a zero memory design for TCP socket in Quark. The design has 2 parts:

% \textbf{Memory mappable TCP socket}: As we discussed in 3.3, TSoR creates 2 fixed size ring buffers (one is read buffer and the other is write buffer) for each TCP socket. The buffers are memory page aligned. TSoR extends sys\_mmap to enable it for TSoR TCP sockets. So the user application can memory map the 2 buffers to user space and then it can use it as user application buffer to avoid extra memory copy.

% \begin{figure}[tbp]
%      \centering
%  \includegraphics[width=\linewidth]{graphs/charts/zero_copy.png}
%  \caption{}
% %  \label{fig::arch}
%  \end{figure}
 
% \textbf{2 more system calls to handle ring buffer head/tail pointers}: The 2 socket kernel buffers are managed as ring buffers with head and tail pointers. TSoR adds 2 system calls to enable user application get/set the head/tail pointer. The 2 system calls signatures are as below.
% \[
% int~sys\_socket\_consume(int: fd, int: count, *iovec: addr, int: flags)
% \]

% This is for the read buffer. It tells Quark Kernel that the $count$ bytes of the read buffer has been consumed by the user application and is Ok to overwrite more data from remote peer. The iovec is an out parameter and returns the iovec array of available data ranges in the read buffer.
% \[
% int~sys\_socket\_produce(int: fd, int: count, *iovec: addr, int: flags)
% \]
% It is for the write buffer. It tells Quark Kernel that the count bytes of the write buffer has been produced by the user application and is ready to send to the remote peer. The iovec is an out parameter and returns the iovec array of free space range.





==> designv2.tex <==
\section{Overview}
\subsection{Design Goal}
TSoR has the following design goals:
% \textbf{Design Goals / Motivation}:eo
\begin{itemize}
\item {\bf High performance container networking for micro-service}: TSoR is designed to transmit TCP traffic through RDMA connection which bypass TCP/IP protocol stack. So it achieves high throughput,  low latency with lower CPU consumption.

\item {\bf Transparency to the application programmer}: TSoR API is compatible with POSIX socket interface. It is designed to significantly improve performance without requiring modifications to applications or containerized application image.

\item {\bf Self-contained container network plugin of Kubernetes environment}:  TSoR is designed to be fully compatible with Kubernetes network model. There should be minimal effort to set up TSoR for existing Kubernetes cluster so that it can be used in existing Kubernetes ecosystem. At the same time, TSoR supports multi-tenant network traffic isolation and provides an efficient network traffic routing solution to address frequent container start up and tear down in serverless computing.
\end{itemize}


\subsection{Requirement and Challenge}

TSoR's goal is to use RDMA as data plan for Kubernetes cluster internal connection. The semantic of TCP socket to transfer data of a local buffer to its peer's remote buffer. RDMA NIC supports to copy data from an application buffer to remote machine's application buffer. The major idea of TSoR data plane is to offload the TCP data transmission to RDMA NIC instead of through TCP/IP protocol stack.  

RDMA supports both unreliable and reliable connection. TSoR choose to use transmit TCP data with RDMA Reliable Connection (RC) so that fully TCP protocol reliability functionality is offloaded to RDMA NIC hardware. 

This is also the design of SMC[] and DirectSocket[], in which TCP connection has one underlying RDMA Reliable Connection, i.e. Reliable Connection (RC) Queue Pair (QP).

From TSoR initial design evaluation work, we found the performance issue for such one TCP connection to one RDMA connection as below. 
\begin{itemize}
\item \textbf{RDMA Reliable Connection scalability}: In a typical cluster environment, the micro-services running on one bar-metal machine might need 1 million TCP connections. Per [], RDMA NIC \textbf{performance will decrease when its Reliable Connection count reach a few hundred}?. 
\item \textbf{RDMA connection setup latency}: The RDMA RC QP connection establishment needs another communication channel, e.g. TCP, to help exchange QP metadata. We measured the latency of creating such RC QP based on TCP connection and found the latency is about 5000 microsecond while a common TCP connection only take about 500 microseconds?. 
\end{itemize}

So it is not practicable for to map one TCP connection to one RDMA Reliable Connection.



\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/requirement.png}
 \caption{TSoR Requirement}
%  \label{fig::arch}
 \end{figure}
TSoR is designed as a Kubernetes Container Network provider. It needs to provide follow connection as Figure\#\#: \circled{1} Intra-node Pod to Pod , \circled{2} Inter-node Pod to Pod , \circled{3} External to Pod (i.e. ingress), \circled{4} Pod to External.

The connection \circled{1} \circled{2}  are Kubernetes cluster internal connection, TSoR will provides a RDMA based TCP connection. The connection \circled{3} \circled{4} are external facing connection, TSoR needs to provide TSoR gateway to handle data transfer. 


\subsection{Architecture}
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TSoRArchv2.png}
 \caption{TSoR Architecture}
%  \label{fig::arch}
 \end{figure}
 
Figure 1 shows the TSoR architecture along with interaction with other entities in a typical micro-service hosting Kubernetes environment. In one TSoR enabled Kubernetes cluster, there will be multiple Cluster Nodes and each Cluster Nodes will composes one RDMA Service, multiple Quark enabled Pods, and one TSoR Gateway.
\begin{itemize}
\item \textbf{RDMA Service}: RDMA service is the TSoR's central component. It implements TSoR Control plane and data plane: 
\begin{itemize}
\item Data plane: RDMA Service the only module talking to RDMA NIC in whole system. All the Quark container of Pods will connect to the Node's RDMA service with shared memory queue and access RDMA NIC through RDMA Service. To mitigate the RDMA connection scalability and setup latency issue, RDMA Service setup one RDMA connection to all other Cluster Node. And all the TCP connection traffic will be multiplex on this RDMA connection.
\item Control plane: RDMA Service will connect to Kubernetes central metadata service API Server to sync up connection related Kubernetes objects metadata such as active Node list. Based on the metadata, RDMA Service know to which Node it sends the TCP traffic. 
\end{itemize}
\item \textbf{TSoR protocol stack}: Quark runtime system call virtualization layer intercept POSIX socket system call and has a network protocol stack to simulate the Linux system call semantic based on host Linux system call interface. TSoR integrates with Quark and take over all the TCP related system call interface and provide a RDMA based simulation implementation. The RDMA based simulation is based on RDMA Service Client, which is the client library to communicate with RDMA Service through the shared memory queue.
\item \textbf{TSoR Gateway}: As traffic internal cluster using TSoR is carried by RDMA network while traffic external traffic is using TCP/IP protocol, a gateway is needed to do transformation between TCP and TSoR for external traffic. A separate section will be used to introduce TSoR gateway and TSoR integration/.
\end{itemize}
 
 
 
% 1) App POSIX Interface and Lightweight VM

% - Quark (syscall) virtualization layer

% - POSIX  

% 2) Data Path: RDMA\_Service

% -control: QP connection setup

% -control: socket connection 

% -data: Data Transfer

% 3) Control Plane: K8S , Ingress/Egress Gateway
\section{TSoR Protocol Stack}
One of the main goal of TSoR is to provide transparency to the application programmer so that applications or containerized application image which uses canonical POSIX socket API[] for TCP related operations can use TSoR without modification. TSoR leverages Quark's system call virtualization layer to achieve this goal.

TSoR introduce a module called TSoR Protocol Stack to replace TCP/IP protocol stack. TSoR protocol stack is responsible for intercepting all POSIX socket calls 


% \section{Control Plane}
% \subsection{Meta Data}

\section{RDMA Service}
RDMA Service is the core module of TSoR, it implements both data plane and control plane. Prior to introduce how RDMA service uses RDMA network to set up TCP socket connection and transmit TCP traffic. We will first introduce some challenges when using RDMA to handle TCP socket, solutions and technical decisions we make and important concepts to be used when building up RDMA service.
\subsection{Technical Decisions}
To transfer TCP traffic using RDMA network, TSoR has following technical choices:
 
 \textbf{RDMA operation choice}: RDMA supports different types operations such as Send, Receive, RDMA Write, etc. We choose RDMA Write With Immediate for TCP traffic transfer. RDMA Write With Immediate operation could copy a user space buffer data to remote machine application buffer as Write operation. And when the copy is done, it will also wake up remote RDMA service with another TSoR defined 32 bits immediate data. The 32 bites immediate data will help TSoR multiplex TCP socket connections over one RDMA QP connection. The choice can achieve lower latency with compromising of the system throughput.


 \textbf{Pod IP address assignment}: TSoR supports multi-tenant container IP address assignment. Different tenants could share the same subnet CIDR. So the assigned address could be expressed as a tube <Tenant ID, IP Address>.  Each Quark container has its tenant id when start up by TSoR. When TSoR allocates IP address for a new container, it will firstly get the container’s Tenant ID and then allocate the free IP address based on that. So far, TSoR used fixed subnet CIDR for all the tenants on one cluster node. The reason of this design is to save IP Address route propagate latency for the frequent container start up and tear down. Because each cluster node has a fixed subnet CIDR for all tenants, RDMA service could create a CIDR to neighbor cluster node mapping. The mapping will only be updated when there is node bootup and shutdown. When RDMA gets a TCP connection request, it can simply look up the map based on  the target IP address’s CIDR to get the remote cluster node no matter which tenant the container belongs to.
 
\subsection{Components and Concepts}
In this section, we describe RDMA service components and concepts. They will be used to illustrate workflows in upcoming sections.

\textbf{rdma\_cm}: RDMA Connection Manager(rdma\_cm) is a component which talks to Kuberntes API server

\textbf{rdma\_srv}: rdma\_srv is a global component inside RDMA service, it maintains global entities such as rdma\_agents, rdma\_connections and rdma\_channels.

\textbf{rdma\_srv\_cli}: Each container including TSoR Ingress and Egress Gateway will set up a RDMA service client (rdma\_srv\_cli). Quark containers and gateways will delegate all TCP socket related operations to rdma\_srv\_cli which then talks to RDMA service via Submit Queues and Complete Queues residing in shared memory between rdma\_srv\_cli and RDMA Service.


\textbf{rdma\_agent}: RDMA Service sets up one RDMA agent (rdm\_agent) for each container and TSoR gateway. rdma\_agent is to pop/push requests which are fed to Submit Queues /Complete Queues between rdma\_srv\_cli and RDMA Service.

\textbf{rdma\_channel}: One rdma\_channel will be created for each TCP socket connection. rdma\_channel is responsible managing ring buffer which is shared between TCP socket and rdma\_channel to prepare data before leveraging RDMA network to send.

\textbf{rdma\_connection}: RDMA Service on each cluster node will set up the RDMA connection (rdma\_connection) between each other node. rdma\_connection is multiplexed for rdma\_channel on current node to send and receive RDMA traffic.

\textbf{rdma\_control\_channel}: One rdma\_control\_channel is created for each rdma\_connection. rdma\_control\_channel is used to exchange rdma\_channel establishment information and other metadata such as remote receive request count.

\textbf{client share region}: ClientShareRegion is a shared memory region between rdma\_srv\_cli and rdma\_agent. cq/sq are lock free shared memory queues to exchange request/response between rdma\_srv\_cli and rdma\_agent. iobuf is a buffer mapped to a socket buffer where the system calls write/read data to/from.
\subsection{Node to Node RDMA QP Connection}
When RDMA service starts up after node joins cluster, it will use following steps to set up RDMA QP Connection:
\begin{enumerate}
\item Start TCP server to listen on a known port to wait for RDMA service on other nodes to connect
\item Retrieve active cluster node list from RDMA CM. Each node entity will has a timestamp which shows it's time to join the cluster.
\item Compare other node timestamp with timestamp on current node. Connect to RDMA service on nodes which timestamp is earlier than current node using TCP socket API.
\item Create rdma\_connection and rdma\_control\_channel using TCP socket connection to exchange RDMA RC QP and rdma\_control\_channel metadata.
\end{enumerate}
\subsection{TCP Socket Connection Establishment}
Canonical TCP uses a three-way handshake to establish a reliable connection which can take time around 300 microseconds. RDMA network has much lower latency, TSoR uses RDMA network(rdma\_control\_channel is used under the hood)to exchange metadata when establishing TCP socket connection following below steps(?? sequential diagram):
\begin{enumerate}
\item {\bf Push Connect Request to submission queue}:rdma\_srv\_cli enqueues one connect request to submission queue between rdma\_srv\_cli and RDMA Service.

\item {\bf Client side rdma\_srv handle Connect Request}:rdma\_srv parses Connect Request, calculates the peer node based on destination container IP in Connect Request, creates rdma\_channel, constructs a connection request and sends it over to peer node via control channel using IB Verb: RDMA Write Immediate.

\item {\bf Server side rdma\_srv handle connection request}:rdma\_srv parse connection request, verify whether there's a container listening on destination {TenantId, IP, port}.
If so, rdma\_srv creates rdma\_channel, enqueue an accept request to Completion Queue of the container which is listening on destination tuple {TenantId, IP, port}. At the same time, rdma\_srv construct connection response request and send it back to client node via RDMA.

\item {\bf Client side rdma\_srv handle connection response}: Client side rdma\_srv parse connection response,save peer rdma\_channel id, construct and enqueue Connect Response to client container

\item {\bf Client side container handle connection response}: Client side container parse connection response, notify application that connection is established and data can be sent. 
\end{enumerate}
We will measure TCP socket connection establishment latency in evaluation section.
\subsection{Data Transfer}
TSoR is using RDMA IB verbs to transfer TCP stream data. RDMA IB verbs can copy user space application data buffers between cluster nodes. RDMA requires the buffer memory to be pre-registered to the RDMA NIC before data transfer. TCP kernel buffer design impact data transfer performance and memory consumption. For each TCP socket, TSoR creates 2 fixed size ring buffers, i.e. read buffer and write buffer, when TCP connections are created for the socket. The Ring buffer memory is shared between the Quark container and RDMA service and  is registered in RDMA. RDMA service uses IB verbs to copy ring buffer data between cluster nodes and synchronize the ring buffer head/tail pointer with Quark container.
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/write_flow.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 
Figure shows TSoR’s TCP data transfer process which has the following steps.
\begin{enumerate}
\item {\bf Ringbuffer Produce}: By this step, SysWrite plays as the producer for the socket buffer and copies data from the application to the writeBuf.

\item {\bf Push Write\_Request to the submit queue}: rdma\_srv\_cli enqueues one write request into the submit queue between rdma\_srv\_cli and rdma\_srv.

\item {\bf RDMA data copy to remote peer}: RDMA\_srv copy the data from local write buffer to remote read buffer with write\_immediate IB verb.

\item {\bf Rdma\_srv processes the received write\_immediate}: The remote rdma\_srv will get notification from RDMA NIC when the data copy is finished. Then RDMA\_srv will notify rdma\_srv\_cli there is data ready for reading in the read buffer by enqueue request in the completion queue between RDMA\_srv and rdma\_srv\_cli.

\item {\bf SysRead consumes the read buffer}: SysRead consumes the read buffer and will copy the data from kernel read buffer to application buffer.
\end{enumerate}
\section{TSoR Integration with Kubernets}
Another main goal of TSoR is to provide a complete self-contained container network plugin working with Kubernetes environment. According to Kubernetes documents[], there are 4 distinct networking problems to address:
\begin{enumerate}
\item Container-to-container communications in same pod.
\item Pod-to-Pod communications.
\item Pod-to-Service communications.
\item External-to-Service communications.
\end{enumerate}
The first 2 communications are already solved by TCP Socket connection and data transfer workflow when introducing RDMA service in previous section. This section will focus on how TSoR implements pod to service and external to service communications.

\subsection{Pod to Service Communication}
In cluster using TSoR, RDMA service will be responsible to route the traffic when pod send request to service.
Rdma\_srv will get service information including the cluster IP and running pods list to serve this service.
When RDMA service get connect request from pod, it will check whether this destination IP address is a pod IP or service IP, if it's service IP, then RDMA service will rewrite the destination IP as one of the pods' ip (currently RDMA service use round robin to pick up the next pod). The following steps including TCP socket connection establishment and data transfer are same as pod to pod communication.
\subsection{External to Service Communication}
Network traffic is transmitted over RDMA network inside cluster using TSoR while traffic outside cluster is over TCP. To make services in cluster available to external world and access services outside of cluster from pod, TSoR gateways are designed and implemented to do transformation between TCP traffic and RDMA traffic. Depending on the traffic direction, TSoR introduces ingress and egress gateway for incoming and outgoing traffic separately.
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TSoRGateway.png}
 \caption{TSoR Gatway Architecture}
%  \label{fig::arch}
 \end{figure}

Figure 4 shows the architecture of both TSoR gateways. 

\textbf{TSoR Ingress Gateway}

TSoR Ingress Gateway is responsible for transforming TCP traffic from outside to RDMA traffic inside cluster using TSoR.
A Kubenetes custom resource definition called TSoRIngress is introduced to set up mapping between external port and internal service. TSoR Ingress gateway will listen on the external port for incoming TCP connection request and traffic. On the other side Ingress gateway uses RDMA Svc Client to talk to RDMA service for TCP traffic and RDMA transformation. 

\textbf{TSoR Egress Gateway}
TSoR Egress Gateway is responsible for transforming RDMA traffic inside cluster using TSoR to outside cluster service.
RDMA Service will forward request to TSoR Egress gateway if traffic destination is not for containers inside cluster. Egress gateway then uses TCP socket to connect to outside cluster service.

With aforementioned mechanisms, TSoR solves all networking problems mentioned in Kubernets cluster. We claim TSoR is a complete self-contained Kubernetes container network plugin which is distinct from other solutions like [].
\subsection{Implementation and Deployment}
Except RDMA Connection Manager, all other modules (RDMA Srv, Ingress, Egress and RDMA stack in Quark container runtime) of TSoR are written in Rust language to achieve efficiency and safety as a system module. The rust code is around 30k line. RDMA Connection Manager is using golang mainly together with Rust building the service client. Total lines are around 10k. 

Currently when deploying a Kuberntes cluster using TSoR, RDMA service, TSoR Ingress and Egress Gateway will be daemon service running on each cluster node. All of them are already built into container images and one single yaml file for all deployoment artifacts are provided for one click deployment.



==> k8sintergration.tex <==
\section{TSoR Integration with Kubernets}
Another main goal of TSoR is to provide a complete self-contained container network plugin working with Kubernetes clusters. According to Kubernetes documents[], there are 4 distinct networking problems to address:
\begin{enumerate}
\item Communication between containers in same Pod.
\item Communication between Pods.
\item Communication between Pod and Service.
\zhao{What is service?}
\item Communication between external entity and Service.
\end{enumerate}

\zhao{title for this process}
All communications can only happen after Pod get a virtual IP address. TSoR is responsible for pod IP assignment. TSoR used fixed subnet CIDR for all the pods on one cluster node. The reason of this design is to eliminate IP Address propagation for routing which is crucial in a environment where pods start up and tear down frequently. Because each cluster node has a fixed subnet CIDR, RDMA service could create a CIDR to peer cluster node mapping. The mapping will only be updated when there is node joining or leaving TSoR cluster. When RDMA gets a TCP connection request, it can simply look up the map based on the destination IP address’s CIDR to get the remote cluster node where the destination pod resides in.
%  \textbf{Pod IP address assignment}: TSoR supports multi-tenant container IP address assignment. Different tenants could share the same subnet CIDR. So the assigned address could be expressed as a tube <Tenant ID, IP Address>.  Each Quark container has its tenant id when start up by TSoR. When TSoR allocates IP address for a new container, it will firstly get the container’s Tenant ID and then allocate the free IP address based on that. So far, TSoR used fixed subnet CIDR for all the tenants on one cluster node. The reason of this design is to save IP Address route propagate latency for the frequent container start up and tear down. Because each cluster node has a fixed subnet CIDR for all tenants, RDMA service could create a CIDR to neighbor cluster node mapping. The mapping will only be updated when there is node bootup and shutdown. When RDMA gets a TCP connection request, it can simply look up the map based on  the target IP address’s CIDR to get the remote cluster node no matter which tenant the container belongs to.
 
% \subsection{Components and Concepts}
% In this section, we describe RDMA service components and concepts. They will be used to illustrate workflows in upcoming sections.

% \textbf{rdma\_cm}: RDMA Connection Manager(rdma\_cm) is a component which talks to Kuberntes API server

% \textbf{rdma\_srv}: rdma\_srv is a global component inside RDMA service, it maintains global entities such as rdma\_agents, rdma\_connections and rdma\_channels.

% \textbf{rdma\_srv\_cli}: Each container including TSoR Ingress and Egress Gateway will set up a RDMA service client (rdma\_srv\_cli). Quark containers and gateways will delegate all TCP socket related operations to rdma\_srv\_cli which then talks to RDMA service via Submit Queues and Complete Queues residing in shared memory between rdma\_srv\_cli and RDMA Service.


% \textbf{rdma\_agent}: RDMA Service sets up one RDMA agent (rdm\_agent) for each container and TSoR gateway. rdma\_agent is to pop/push requests which are fed to Submit Queues /Complete Queues between rdma\_srv\_cli and RDMA Service.

% \textbf{rdma\_channel}: One rdma\_channel will be created for each TCP socket connection. rdma\_channel is responsible managing ring buffer which is shared between TCP socket and rdma\_channel to prepare data before leveraging RDMA network to send.

% \textbf{rdma\_connection}: RDMA Service on each cluster node will set up the RDMA connection (rdma\_connection) between each other node. rdma\_connection is multiplexed for rdma\_channel on current node to send and receive RDMA traffic.

% \textbf{rdma\_control\_channel}: One rdma\_control\_channel is created for each rdma\_connection. rdma\_control\_channel is used to exchange rdma\_channel establishment information and other metadata such as remote receive request count.

% \textbf{client share region}: ClientShareRegion is a shared memory region between rdma\_srv\_cli and rdma\_agent. cq/sq are lock free shared memory queues to exchange request/response between rdma\_srv\_cli and rdma\_agent. iobuf is a buffer mapped to a socket buffer where the system calls write/read data to/from.

The first 2 communications are already illustrated by TCP socket connection establishment and data transfer workflow. This section will focus on how TSoR implements pod to service and external to service communications.

\subsection{Pod to Service Communication}
In cluster using TSoR, RDMA service is responsible for routing the traffic when pod send request to service. RDMA Service will get service information including the cluster IP and running pods list to serve this service. When RDMA service get connect request from pod, it will check whether the destination IP address is a pod IP or service IP, if it's service IP, then RDMA service will rewrite the destination IP as one of the pods' ip (currently RDMA service use round robin to pick up the next pod). The following steps including TCP socket connection establishment and data transfer are same as pod to pod communication.
\subsection{External to Service Communication}
Network traffic is transmitted over RDMA network inside cluster using TSoR while traffic outside cluster is over TCP. To make services in cluster available to external world and access services outside of cluster from pod, TSoR uses gateways to do transformation between TCP traffic and RDMA traffic.
% \begin{figure}[tbp]
%      \centering
%  \includegraphics[width=\linewidth]{graphs/charts/TSoRGateway.png}
%  \caption{TSoR Gatway Architecture}
% %  \label{fig::arch}
%  \end{figure}

% Figure 4 shows the architecture of both TSoR gateways. 

% \textbf{TSoR Ingress Gateway}

% TSoR Ingress Gateway is responsible for transforming TCP traffic from outside to RDMA traffic inside cluster using TSoR.
% A Kubenetes custom resource definition called TSoRIngress is introduced to set up mapping between external port and internal service. TSoR Ingress gateway will listen on the external port for incoming TCP connection request and traffic. On the other side Ingress gateway uses RDMA Svc Client to talk to RDMA service for TCP traffic and RDMA transformation. 

% \textbf{TSoR Egress Gateway}
% TSoR Egress Gateway is responsible for transforming RDMA traffic inside cluster using TSoR to outside cluster service.
% RDMA Service will forward request to TSoR Egress gateway if traffic destination is not for containers inside cluster. Egress gateway then uses TCP socket to connect to outside cluster service.

% With aforementioned mechanisms, TSoR solves all networking problems mentioned in Kubernets cluster. We claim TSoR is a complete self-contained Kubernetes container network plugin which is distinct from other solutions like [].
% \subsection{Implementation and Deployment}
% Except RDMA Connection Manager, all other modules (RDMA Srv, Ingress, Egress and RDMA stack in Quark container runtime) of TSoR are written in Rust language to achieve efficiency and safety as a system module. The rust code is around 30k line. RDMA Connection Manager is using golang mainly together with Rust building the service client. Total lines are around 10k. 

% Currently when deploying a Kuberntes cluster using TSoR, RDMA service, TSoR Ingress and Egress Gateway will be daemon service running on each cluster node. All of them are already built into container images and one single yaml file for all deployoment artifacts are provided for one click deployment.

==> workflow.tex <==
\section{Workflow}

\zhao{section title}

This section will present important workflows including node to node RDMA Connection establishment, TCP socket connection establishment and TCP socket data transfer with TSoR.
\subsection{Pre-established RDMA Connection}
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/QPConnection.png}
 \caption{RDMA Connection Establishment}
%  \label{fig::arch}
 \end{figure}
When RDMA service starts up after node joins TSoR cluster, it will establish RDMA Connections to all its peer Nodes in the cluster. All the TCP traffic will be multiplexed over this RDMA connection to migrate the RDMA Connection scalability issue. At the same time TCP connection establishment is also using this reliable and low latency RDMA Connection, so that TSoR can achieve low latency TCP connection establishment.

Figure [] shows the process to set up node to node RDMA connection which is summarized as following:
\begin{enumerate}
\item Start TCP server to listen on a known port to wait for RDMA service on other nodes to connect;
\item Retrieve active cluster node list from the cluster orchestration control plane;
\item Setup TCP connection with the peer nodes which join TSoR Cluster earlier than current node;
\item Setup RDMA connections with peer nodes by exchanging RDMA metadata over the TCP connection;
\end{enumerate}

\subsection{2-way Connection Handshake Establishment}
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/TCPWorkflow.png}
 \caption{TCP Socket Workflow}
%  \label{fig::arch}
 \end{figure}
Canonical TCP/IP protocol stack uses a 3-way handshake to establish a TCP connection which usually takes around hundreds of microseconds to complete. TSoR's TCP connection establishment is based on reliable underlying RDMA Connection. So we choose 2-way handshake for connection establishment, top half part of figure [] shows the process which is also summarized as following steps:
\begin{enumerate}
\item  \textbf{User application make a TCP connect call}: The Quark runtime will intercept the connect call and TSoR client will use the connect call parameters such as socket and destination IP address and port to process it; 
\item \textbf{TSoR Client send TCP Connect Request to RDMA Service}: TSoR Client en-queue one TCP connect request in Submission Queue between TSoR Client and RDMA Service.

\item \textbf{Client side RDMA Service send RDMA Channel connection request to server side RDMA Service}: Client side RDMA Service parses TCP connect request, retrieves the peer node based on destination container IP, create a RDMA Channel, constructs a RDMA Channel connection request and sends it to server side RDMA service via RDMA Control Channel;

\item \textbf{Server side RDMA Service en-queue TCP accept request}: Server side RDMA Service will create a RDMA Channel, construct RDMA Channel connection response request and send it back to Client side RDMA Service via RDMA Control Channel. After that, Server side RDMA Service en-queue TCP accept request to Completion Queue of the server container's TSoR Client.

\item \textbf{Client side RDMA Service notify container TSoR client}: Client side RDMA Service parse RDMA Channel connection response from Server side RDMA Service, en-queue an TCP accept request to Completion Queue of the client container's TSoR Client.

\item \textbf{Client side TSoR client notify user application}: Client side TSoR client notifies application that connection is established and is ready for data transmission. 
\end{enumerate}

 TSoR uses two-ways  handshake instead of three-way as the TSoR's TCP connection is established over reliable RDMA Connection. As the RDMA latency is low, TSoR's TCP connection establishment latency is lower than TCP/IP protocol stack.

\subsection{RDMA based TCP Data Transmission}
\zhao{I think we should move this subsection to 4.1}
TSoR is designed to achieve high network performance as it transmits TCP stream data over underlying RDMA Connection. RDMA can write user space application data to remote node application data buffer directly without involving host OS kernel. The data write is done by RDMA NIC hardware bypass the OS kernel so that it has high performance and low latency with less CPU usage.

RDMA requires the buffer memory to be pre-registered to the RDMA NIC before data transfer. TCP kernel buffer design impact data transfer performance and memory consumption. For each TCP socket, TSoR creates 2 fixed size ring buffers, i.e. read buffer and write buffer, when TCP connections are established for the socket. The ring buffer memory is shared between Quark container and RDMA service and pre-registered with RDMA. RDMA service uses IB verbs to transfer ring buffer data and synchronize buffer capacity with peer node. At the same time ring buffer head and tail pointer are synchronized between TSoR client and RDMA service using shared buffer metadata.
\begin{figure}[tbp]
     \centering
 \includegraphics[width=\linewidth]{graphs/charts/write_flow.png}
 \caption{}
%  \label{fig::arch}
 \end{figure}
 
Bottom half part of figure [] and figure [] shows TSoR’s TCP data transfer process which has the following steps.
\begin{enumerate}
\item {\bf Application makes write call}: Quark runtime intercepts the system call, TSoR Client plays as the producer for the socket buffer and copies data from the application into the write buffer.

\item {\bf Push Write Request to the Submission queue}: TSoR client en-queues one write request into the submission queue shared between TSoR client and RDMA service.

\item {\bf Transmit data to peer over RDMA}: RDMA Service uses RDMA IB verb to send data from write buffer to remote node over RDMA

\item {\bf Handle received data over RDMA}: RDMA service on remote node will get notification when RDMA completes the data transfer. Then RDMA Service will notify TSoR Client there is data ready for reading in the read buffer by enqueue request in the completion queue between RDMA Service and TSoR Client.

\item {\bf Read data in read buffer}: TSoR consumes data in the read buffer by copying the data from kernel read buffer to application buffer. Application read call either return or continue reading more data.
\end{enumerate}
